COSMOS: 3D weak lensing and the growth of structure

We present a three dimensional cosmic shear analysis of the Hubble Space Telescope COSMOS survey, the largest ever optical imaging program performed in space. We have measured the shapes of galaxies for the tell-tale distortions caused by weak gravitational lensing, and traced the growth of that signal as a function of redshift. Using both 2D and 3D analyses, we measure cosmological parameters Omega_m, the density of matter in the universe, and sigma_8, the normalization of the matter power spectrum. The introduction of redshift information tightens the constraints by a factor of three, and also reduces the relative sampling (or "cosmic") variance compared to recent surveys that may be larger but are only two dimensional. From the 3D analysis, we find sigma_8*(Omega_m/0.3)^0.44=0.866+^0.085_-0.068 at 68% confidence limits, including both statistical and potential systematic sources of error in the total budget. Indeed, the absolute calibration of shear measurement methods is now the dominant source of uncertainty. Assuming instead a baseline cosmology to fix the geometry of the universe, we have measured the growth of structure on both linear and non-linear physical scales. Our results thus demonstrate a proof of concept for tomographic analysis techniques that have been proposed for future weak lensing surveys by a dedicated wide-field telescope in space.

==> build <==
latex ms.tex ; latex ms.tex ; latex ms.tex
dvips -t letter ms.dvi -o ms.ps
#dvipdf ms.dvi ms.pdf
\rm ms.log
\rm ms.dvi
\rm ms.aux

